Dialog Flow Induction for Constrainable LLM-Based Chatbots

LLM-driven dialog systems are used in a diverse set of applications, ranging from healthcare to customer service. However, given their generalization capability, it is difficult to ensure that these chatbots stay within the boundaries of the specialized domains, potentially resulting in inaccurate information and irrelevant responses. This paper introduces an unsupervised approach for automatically inducing domain-specific dialog flows that can be used to constrain LLM-based chatbots. We introduce two variants of dialog flow based on the availability of in-domain conversation instances. Through human and automatic evaluation over various dialog domains, we demonstrate that our high-quality data-guided dialog flows achieve better domain coverage, thereby overcoming the need for extensive manual crafting of such flows.

==> sections/related_work.tex <==
\section{Related Work}

%\gokhan{My high level comment is that, as I mentioned in our meeting, you confuse dialogue schema with dialogue flow. Here you also includedd dialogue schema induction papers, like clustering the ontology, finding slots, etc., whereas you are inducing the dialogue flow. Please fix your terminology. Flow is flow, schema is schema.}

%\heng{a main problem on the current writing is that it's not clear which ideas are from you vs. from previous work. need to be structured in a better way. Currently the method section includes a lot of generic motivations and challenge discussions}

\subsection{Flow Induction}



%Parallels can be drawn between dialog flow induction and event schema induction~\cite{Li2020c, schemagraphauto2022, hierarchicalschema2023}. Event schema induction aims to depict the typical structure of complex news events based on historical occurences, as a means to analyze, predict, and possibly intervene in the ongoing events~\cite{Li2021b}. Event schema induction is typically done in the news domain, wherein extensive predefined ontologies~\cite{ace2005} are available to map the schema node to an event type. On the other hand, dialog flows have nodes with free-form action labels that are unconstrained, as different dialog domains comprise different tasks. 


%In contrast, dialog flows need to consider dynamic user intents, and thereby have multiple pathways to achieve objectives to accommodate the variability in user preferences for identical tasks.
%In contrast, dialog flows need to account for dynamic user intents by considering multiple trajectories to reach the goal, as user preferences can be different in different instances of the same task.

\begin{comment}

\subsection{Constraining LLM-based Dialog}

\revanth{This section should describe what prior approaches to using bots with dialog flows/schemas have done. Then discuss differences from our approach, in that it is unsupervised, uses feedback which can be extended to human-in-loop settings, along with added customizability}

Early dialog systems heavily relied on expensive rule-based approaches, such as finite state machines for turns \cite{raux-eskenazi-2009-finite} and decision trees \cite{sato2002learning}. Such systems suffered from limited flexibility and were restricted to scripted conversations \cite{10.1007/978-3-642-04208-9_3} \cite{Ward_DeVault_2017}. The introduction of robust machine learning tasks then paved the way for more flexible and understanding systems. For example, early dialog state tracking systems \cite{Stolcke_2000} and the incorporation of n-gram algorithms \cite{dialog2006} significantly improved the flexibility of dialog systems. However, recent advancements in generative large language models have pushed the boundaries of what is possible. Instruction-tuned LLMs, specifically, are able to handle complex meta-tasks that provide dramatic improvements in dialog systems, such as \cite{mishra2024characterizing}, text classification for strong dialog state tracking \cite{sun2023text}, and flexibility for different instruction in different domains \cite{yang2023empower}.

%Before major advancements in LLMs changed dialog systems, task-oriented dialog relied on rule-based approaches that could only produce scripted dialog. These systems followed a finite state machine of possible bot responses, which meant significant manual effort was required for each individual domain, and conversations often were "unnatural" as only scripted responses were produced. Recently, new approaches to task-oriented dialog systems leverage instruction-tuned LLMs to produce "natural" bot responses to any user inquiry. However, these current methods often fail at extraneous user input and entertain irrelevant conversations. In contrast, our approach of constraining LLMs to a automatically generated dialog schema allows for both natural responses that encourage users to interact and controlled conversations that stay on-track.

In practical applications, manually designing dialog can be error-prone, laborious, iterative, and slow, especially when the schema is complicated \cite{yu2022unsupervised}. 



\heng{the following paragraphs are too detailed, compress them into a few shorter paragraphs}

In this section we introduce some of the prior work on automatic schema induction. An unsupervised methodology introduced by \citet{yu2022unsupervised}. utilizes unsupervised span extraction and a nuanced clustering technique for slot type identification, circumventing the need for manual annotations and showcasing potential in scalable applications like call centers. Despite its efficiency, this method's dependence on pre-existing models and probabilistic context-free grammars limits its adaptability across various domains.

The second approach, as elucidated by \citet{chen2015learning} and \citet{hudevcek2023llms}, revolves around the use of annotated FrameNet for semantic frame labeling in raw utterances. This method involves the design of semantic grammars based on generic contexts which may encompass frames pertinent to the target domain, as well as those that are not. While this approach is advantageous for its unsupervised nature, one significant challenge is its potential inability to identify all relevant slots, particularly those not predefined in FrameNet, like specific internet-related terms.

% \textbf{Unsupervised Slot Schema Induction}: 
% The approach by \cite{yu2022unsupervised}, and others involves an unsupervised span extraction stage followed by a coarse-to-fine clustering. This method primarily focuses on extracting spans from user utterances and clustering them into groups that correspond to slot types, such as “internet” with values like “with wifi”, “no wifi”, etc. These clusters are then mapped to slot type labels for applications in dialog state tracking and response generation. The key advantage of this method is its independence from labor-intensive manual annotations, making it scalable and efficient for real-world applications like call centers. However, this approach still relies on pre-trained language models and probabilistic context-free grammar structures, which may limit its adaptability to new tasks and domains. 

% \textbf{Schema Induction for Dialog Using FrameNet}: Another line of work, as discussed by \cite{chen2015learning} and \cite{hudevcek2023llms}, focuses on using annotated FrameNet to label semantic frames for raw utterances. This method designs semantic grammars based on generic contexts, which may include frames relevant to the target domain as well as irrelevant ones. The limitation here is that it might not extract all relevant slots, especially those not defined in FrameNet, like “internet”. Moreover, this approach, despite its unsupervised nature, often requires manual tuning and may not be adaptable to diverse domains or large datasets.

Unlike previous methods that partially depend on predefined structures or models, our approach is completely unsupervised. It does not rely on any pre-trained models or manual annotations, making it uniquely adaptable to a wide range of domains and tasks.Our method extends to include feedback, which can be either human-in-the-loop or customized according to the domain-specific needs. This adaptability is a significant departure from prior methods that often lack the flexibility to incorporate real-time or domain-specific feedback. The unsupervised nature of our approach, coupled with its feedback mechanisms, offers unparalleled customizability and scalability. This makes it particularly suitable for today's dynamic and varied dialog contexts, where the ability to quickly adapt and scale is crucial.
\dilek{you need more sections/citations for this section. For example, you need to discuss learning dialogue policies, work that aims to discover user intents and concepts from data. Some related work we were mentioning: pls check the tex file, I added pointers to papers there, in the comments below:}

% https://www.researchgate.net/profile/Dilek-Hakkani-Tur/publication/305719953_Clustering_Novel_Intents_in_a_Conversational_Interaction_System_with_Semantic_Parsing/links/579b7f7008ae5d5e1e137f89/Clustering-Novel-Intents-in-a-Conversational-Interaction-System-with-Semantic-Parsing.pdf,
% \cite{hakkaniclustering}
% https://arxiv.org/pdf/1904.08524.pdf, 
% \cite{vedula2019open}
% https://arxiv.org/pdf/2012.15543.pdf, 
% \cite{xu2020discovering}
% https://www.lti.cs.cmu.edu/sites/default/files/research/thesis/2008/ananlada_chotimongkol_learning_the_structure_of_task-oriented_conversations_from_the_corpus_of_in-domain_dialogs.pdf
% \cite{Chotimongkol2008LearningTS} 
\end{comment}
